What Makes Transfer Learning Work For Medical Images: Feature Reuse & Other Factors

Transfer learning is a standard technique to transfer knowledge from one domain to another. For applications in medical imaging, transfer from ImageNet has become the de-facto approach, despite differences in the tasks and image characteristics between the domains. However, it is unclear what factors determine whether - and to what extent - transfer learning to the medical domain is useful. The long-standing assumption that features from the source domain get reused has recently been called into question. Through a series of experiments on several medical image benchmark datasets, we explore the relationship between transfer learning, data size, the capacity and inductive bias of the model, as well as the distance between the source and target domain. Our findings suggest that transfer learning is beneficial in most cases, and we characterize the important role feature reuse plays in its success.

==> tables/deit-model-capacaty-details.tex <==

\begin{tabular}{l|l}
\textbf{WT-ST Config name} & \textbf{Block used for WT-ST} \\ \hline
WT-ST-0/14        & ---                  \\ \hline
WT-ST-1/13        & patch\_embed         \\ \hline
WT-ST-2/12        & block 0              \\ \hline
WT-ST-3/11        & block 1              \\ \hline
WT-ST-4/10        & block 2              \\ \hline
WT-ST-5/9         & block 3              \\ \hline
WT-ST-6/8         & block 4              \\ \hline
WT-ST-7/7         & block 5              \\ \hline
WT-ST-8/6         & block 6              \\ \hline
WT-ST-9/5         & block 7              \\ \hline
WT-ST-10/4        & block 8              \\ \hline
WT-ST-11/3        & block 9              \\ \hline
WT-ST-12/2        & block 10             \\ \hline
WT-ST-13/1        & block 11             \\ \hline
WT-ST-14/0        & layer norm          
\end{tabular}
\caption{Details of the layers of the {\deitBase} and {\deitTiny} models used for the WT-ST experiments.}
\label{tab:deit_capacity_layer_detials}

==> tables/deit-s-details.tex <==
% \begin{tabular}{l@{\hspace{2mm}}l@{\hspace{1mm}}l}
\begin{tabular}{lll}
\toprule
\textbf{WT-ST-n/m} & 
\textbf{Modules} & 
\textbf{Intermediate layers} 
\\
\midrule

\multirow{1}{*}{WT-ST-0/14} &  &
\\[0.5em]
\multirow{1}{*}{WT-ST-1/13} &
Patchifier &
Conv2d
\\[0.5em]
\multirow{2}{*}{WT-ST-2/12} &
\multirow{2}{*}{Block 1} &
Block 1 -- Attention \\ & &
Block 1 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-3/11} &
\multirow{2}{*}{Block 2} &
Block 2 -- Attention \\ & &
Block 2 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-4/10} &
\multirow{2}{*}{Block 3} &
Block 3 -- Attention \\ & &
Block 3 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-5/9} &
\multirow{2}{*}{Block 4} &
Block 4 -- Attention \\ & &
Block 4 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-6/8} &
\multirow{2}{*}{Block 5} &
Block 5 -- Attention \\ & &
Block 5 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-7/7} &
\multirow{2}{*}{Block 6} &
Block 6 -- Attention \\ & &
Block 6 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-8/6} &
\multirow{2}{*}{Block 7} &
Block 7 -- Attention \\ & &
Block 7 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-9/5} &
\multirow{2}{*}{Block 8} &
Block 8 -- Attention \\ & &
Block 8 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-10/4} &
\multirow{2}{*}{Block 9} &
Block 9 -- Attention \\ & &
Block 9 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-11/3} &
\multirow{2}{*}{Block 10} &
Block 10 -- Attention \\ & &
Block 10 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-12/2} &
\multirow{2}{*}{Block 11} &
Block 11 -- Attention \\ & &
Block 11 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-13/1} &
\multirow{2}{*}{Block 12} &
Block 12 -- Attention \\ & &
Block 12 -- MLP
\\[0.5em]
\multirow{1}{*}{WT-ST-14/0} &
Layer norm &
\\[0.5em]

\bottomrule
\end{tabular}


==> tables/inception-details.tex <==
% \begin{tabular}{l@{\hspace{2mm}}l@{\hspace{1mm}}l}
\begin{tabular}{lll}
\toprule
\textbf{WT-ST-n/m} & 
\textbf{Modules} & 
\textbf{Intermediate layers} 
\\
\midrule

\multirow{1}{*}{WT-ST-0/7} &  &
\\[0.5em]
\multirow{1}{*}{WT-ST-1/6} &
Layer 1 &
Conv2d
\\[0.5em]
\multirow{2}{*}{WT-ST-2/5} &
\multirow{2}{*}{Layer 2} &
Layer 2, Conv2d \\ & &
Layer 2, Conv2d
\\[0.5em]
\multirow{1}{*}{WT-ST-3/4} &
Layer 3 &
Conv2d
\\[0.5em]
\multirow{1}{*}{WT-ST-4/3} &
Layer 4 &
Conv2d
\\[0.5em]
\multirow{3}{*}{WT-ST-5/2} &
\multirow{3}{*}{Stage 1} &
Stage 1, Block 1 -- Type A \\ & &
Stage 1, Block 2 -- Type A \\ & &
Stage 1, Block 3 -- Type A
\\[0.5em]
\multirow{5}{*}{WT-ST-6/1} &
\multirow{5}{*}{Stage 2} &
Stage 2, Block 1 -- Type B \\ & &
Stage 2, Block 2 -- Type C \\ & &
Stage 2, Block 3 -- Type C \\ & &
Stage 2, Block 4 -- Type C \\ & &
Stage 2, Block 5 -- Type C 
\\[0.5em]
\multirow{3}{*}{WT-ST-7/0} &
\multirow{3}{*}{Stage 3} &
Stage 3, Block 1 -- Type D \\ & &
Stage 3, Block 2 -- Type E \\ & &
Stage 3, Block 3 -- Type E
\\[0.5em]

\bottomrule
\end{tabular}


==> tables/resnet-model-capacaty-details.tex <==

\begin{tabular}{l|l}
\textbf{WT-ST Config name} & \textbf{Block used for WT-ST} \\ \hline
WT-ST-0/6 & ---     \\ \hline
WT-ST-1/5 & conv 1  \\ \hline
WT-ST-2/4 & bn 1    \\ \hline
WT-ST-3/3 & layer 1 \\ \hline
WT-ST-4/2 & layer 2 \\  \hline
WT-ST-5/1 & layer 3 \\  \hline
WT-ST-6/0 & layer 4 \\
\end{tabular}
\caption{Details of the layers of the {\resnetOneFiftyTwo} and {\resnetEighteen} models used for the WT-ST experiments.}
\label{tab:res_capacity_layer_detials}

==> tables/resnet50_details.tex <==
% \begin{tabular}{l@{\hspace{2mm}}l@{\hspace{1mm}}l}
\begin{tabular}{lll}
\toprule
\textbf{WT-ST-n/m} & 
\textbf{Modules} & 
\textbf{Intermediate layers} 
\\
\midrule

\multirow{1}{*}{WT-ST-0/6} &  &
\\[0.5em]
\multirow{1}{*}{WT-ST-1/5} &
Layer 1 &
Conv2d
\\[0.5em]
\multirow{1}{*}{WT-ST-2/4} &
Norm layer (BN) & 
\\[0.5em]
\multirow{3}{*}{WT-ST-3/3} &
\multirow{3}{*}{Stage 1} &
Stage 1, Block 1 \\ & &
Stage 1, Block 2 \\ & &
Stage 1, Block 3
\\[0.5em]
\multirow{4}{*}{WT-ST-4/2} &
\multirow{4}{*}{Stage 2} &
Stage 2, Block 1 \\ & &
Stage 2, Block 2 \\ & &
Stage 2, Block 3 \\ & &
Stage 2, Block 4 
\\[0.5em]
\multirow{6}{*}{WT-ST-5/1} &
\multirow{6}{*}{Stage 3} &
Stage 3, Block 1 \\ & &
Stage 3, Block 2 \\ & &
Stage 3, Block 3 \\ & &
Stage 3, Block 4 \\ & &
Stage 3, Block 5 \\ & &
Stage 3, Block 6
\\[0.5em]
\multirow{3}{*}{WT-ST-6/0} &
\multirow{3}{*}{Stage 4} &
Stage 4, Block 1 \\ & &
Stage 4, Block 2 \\ & &
Stage 4, Block 3
\\[0.5em]

\bottomrule
\end{tabular}


==> tables/swin-details.tex <==
% \begin{tabular}{l@{\hspace{2mm}}l@{\hspace{1mm}}l}
\begin{tabular}{lll}
\toprule
\textbf{WT-ST-n/m} & 
\textbf{Modules} & 
\textbf{Intermediate layers} 
\\
\midrule

\multirow{1}{*}{WT-ST-0/14} &  &
\\[0.5em]
\multirow{1}{*}{WT-ST-1/13} &
Patchifier &
Conv2d
\\[0.5em]
\multirow{2}{*}{WT-ST-2/12} &
\multirow{2}{*}{Stage 1, Block 1} &
Stage 1, Block 1 -- Attention \\ & &
Stage 1, Block 1 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-3/11} &
\multirow{2}{*}{Stage 1, Block 2} &
Stage 1, Block 2 -- Attention \\ & &
Stage 1, Block 2 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-4/10} &
\multirow{2}{*}{Stage 2, Block 1} &
Stage 2, Block 1 -- Attention \\ & &
Stage 2, Block 1 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-5/9} &
\multirow{2}{*}{Stage 2, Block 2} &
Stage 2, Block 2 -- Attention \\ & &
Stage 2, Block 2 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-6/8} &
\multirow{2}{*}{Stage 3, Block 1} &
Stage 3, Block 1 -- Attention \\ & &
Stage 3, Block 1 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-7/7} &
\multirow{2}{*}{Stage 3, Block 2} &
Stage 3, Block 2 -- Attention \\ & &
Stage 3, Block 2 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-8/6} &
\multirow{2}{*}{Stage 3, Block 3} &
Stage 3, Block 3 -- Attention \\ & &
Stage 3, Block 3 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-9/5} &
\multirow{2}{*}{Stage 3, Block 4} &
Stage 3, Block 4 -- Attention \\ & &
Stage 3, Block 4 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-10/4} &
\multirow{2}{*}{Stage 3, Block 5} &
Stage 3, Block 5 -- Attention \\ & &
Stage 3, Block 5 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-11/3} &
\multirow{2}{*}{Stage 3, Block 6} &
Stage 3, Block 6 -- Attention \\ & &
Stage 3, Block 6 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-12/2} &
\multirow{2}{*}{Stage 4, Block 1} &
Stage 4, Block 1 -- Attention \\ & &
Stage 4, Block 1 -- MLP
\\[0.5em]
\multirow{2}{*}{WT-ST-13/1} &
\multirow{2}{*}{Stage 4, Block 2} &
Stage 4, Block 2 -- Attention \\ & &
Stage 4, Block 2 -- MLP
\\[0.5em]
\multirow{1}{*}{WT-ST-14/0} &
Layer norm &
\\[0.5em]

\bottomrule
\end{tabular}

